A Reduced Order Iterative Linear Quadratic Regulator (ILQR) Technique for the Optimal Control of Nonlinear Partial Differential Equations

In this paper, we introduce a reduced order model-based reinforcement learning (MBRL) approach, utilizing the Iterative Linear Quadratic Regulator (ILQR) algorithm for the optimal control of nonlinear partial differential equations (PDEs). The approach proposes a novel modification of the ILQR technique: it uses the Method of Snapshots to identify a reduced order Linear Time Varying (LTV) approximation of the nonlinear PDE dynamics around a current estimate of the optimal trajectory, utilizes the identified LTV model to solve a time-varying reduced order LQR problem to obtain an improved estimate of the optimal trajectory along with a new reduced basis, and iterates till convergence. The convergence behavior of the reduced order approach is analyzed and the algorithm is shown to converge to a limit set that is dependent on the truncation error in the reduction. The proposed approach is tested on the viscous Burger's equation and two phase-field models for microstructure evolution in materials, and the results show that there is a significant reduction in the computational burden over the standard ILQR approach, without significantly sacrificing performance.

==> Acknowledgements.tex <==
\section{Acknowledgements}
This work was partially supported by inputs and moral support by M.N.G. Mohamed, which helped the author overcome his crippling existential crisis.
Also, coffee helped.

==> Algorithm.tex <==
\section{The Reduced Order ILQR Algorithm}
\textcolor{red}{You should describe the main steps of ILQR and then how you modify the steps to obtain your RO-ILQR algorithm, currently your algorithm is indecipherable!}
The ILQR algorithm as it stands unfortunately faces the same issue of the Curse of Dimensionality when we scale the optimal control problems of PDEs to realistic resolutions. This is especially significant in the LTV system identification about a trajectory. 

\textcolor{red}{you should briefly describe ILQR here in words.} Let the PDE be discretized and modeled as an $N$-dimensional set of ODEs, with $p$ control inputs. The corresponding LTV system around an arbitrary trajectory is given by:

% Given a trajectory $\{x_t\}_{t=0}^T$ corresponding to control input $\{u_t\}_{t=0}^{T-1}$, we can use input-output perturbation and a Linear Least Squares method to estimate the LTV system given as

\begin{equation}
    \delta x_{t+1} = A_t \delta x_t + B_t \delta u_t
\end{equation}
where $A_t\in \mathbb{R}^{N\times N}$ and $B_t\in \mathbb{R}^{N\times p}$. To estimate the parameters $A_t$ and $B_t$, we can use input-output perturbation and a Linear Least Squares approach. Thus, we need at least $O(N+p)$ rollouts to identify the LTV system parameters.
\textcolor{red}{Explain how you would estimate these parameters using rollouts.}\\
When we scale up the PDE discretization, the increase in dimensionality leads to a quadratic increase in the number of parameters needed to be identified, thus requiring increasingly large number of samples to do so. Thus, the LTV system identification takes up an inordinate amount of time, which makes the ILQR approach intractable for PDEs. thus, in the following, we propose a POD based LTV identification technique that drastically reduces the computational burden of the LTV identification.

\textcolor{red}{The language and description in the following is too loose, you are writing a scientific paper! Please carefully describe the different steps below ``in the body of the paper", not in some algorithm!}

\subsection{Reduced Order LTV System}
\input{PerturbationModel.tex} 

\subsection{Compensation for basis change}
\textcolor{red}{What follows in IV B and C reads like gibberish, please describe carefully in terms of the iLQR algorithm steps.}
The reduced order basis used to project the dynamics and find the local LTV approximation can change significantly when changing the original trajectory, thus rendering the reduced order model invalid. For small perturbations to the trajectory, we can use the same set of basis for a decent approximation, but need to compensate for larger perturbations, such as the new trajectory after an iteration of the ILQR algorithm. 
In order to keep the model up-to-date with the new trajectory, we implement a repeated use of the snapshot-POD to compute the basis corresponding to that trajectory.
The new projection to the reduced order, LTV system identification and computations within the iterate thus make use of the shifted basis.

\subsection{Backward pass}
From the reduced order approximation of the initial trajectory, we can write the Bellman equation
\begin{equation*}
    J_t (\Phi \alpha_t)= \min_{u_t} \{c_t(\Phi \alpha_t, u_t)+J_{t+1} (\Phi \alpha_{t+1})
\end{equation*}
where $\alpha_{t+1}$ can be retrieved from the reduced order dynamics in Eq. 4. We can thus write the perturbed


% The backward-pass for the roILQR algorithm is summarized in Algorithm \ref{roILQR3}.

Thus, we summarize the roILQR algorithm as given in Algorithms \ref{roILQR1}, \ref{roILQR2} and \ref{roILQR3}.

\begin{algorithm}
  \caption{\strut Reduced-order ILQR with Shifting Basis}
  
  {\bf Initialization:} Set state $x = x_0$, initial guess $u^0_{0:T-1}$, line search parameter $\alpha = 1$, regularization $\mu = 10^{-6}$, iteration counter $k = 0$, convergence coefficient $\epsilon = 0.001$, line search threshold $\sigma_1=0.3$.\\
  
  Initial trajectory: $\{x_t^0\}_{t=0}^T=simulate\_forward\_step(x_0,u^0_{0:T-1})$\\
  Initialize the basis: $\Phi^{(0)} = snapshot\_pod(\{x_t^0\}_{t=0}^T)$\\
  \While {$cost_{k}/cost_{k-1} < 1 - \epsilon$}{
  \CommentSty{/* backward pass */}\\
  \{$k^{k}_{0:T-1}, K^{k}_{0:T-1}$\} $=$ backward\_pass()\\
  \CommentSty{/* forward pass */}\\
  Initialize $z=1$.\\
      \While{$z < \sigma_1$}{
            Reduce $\alpha$, \\
            $u^{k+1}_{0:T-1}$, $cost_k$, $\Delta cost(\alpha)$ $=$ forward\_pass($u^{k}_{0:T-1},\{k^{k}_{0:T-1}, K^k_{0:T-1}\}$),\\
            $z=(cost_k-cost_{k-1})/\Delta cost(\alpha),$\\
        }
        $k \leftarrow k + 1.$
      }{
      $\bar{u}_{0:T-1} \gets u^{k+1}_{0:T-1}$\\
  }
  
  
  
  \label{roILQR1}
\end{algorithm}

\begin{algorithm}
% \footnotesize
 \caption{\strut Forward Pass}
  {\bf Input:} Previous iteration nominal trajectory - $u^{k}_{0:T-1}$, iLQR gains - $\{k_{0:T-1}, K_{0:T-1}\}$.\\
  Start from $t = 0$, $cost = 0$, $\Delta cost(\alpha)=0$, $\bar{x}_0 = x_0$.\\
  \While {$t < T$}{
    \begin{equation*}
    \begin{split}
        u^{k+1}_{t} &= u_t^{k} + \alpha k_t + K_{t} ({x^{k+1}_t} - {x_t^{k}}),\\
        {x^{k+1}_{t+1}} &= simulate\_forward\_step(x^{k+1}_{t}, {u_t^{k+1}}),\\
        cost &= cost + incremental\_cost({x^{k+1}_{t}}, {u_t^{k+1}}),\\
        \end{split}
    \end{equation*}
    $t \leftarrow t + 1$. 
    }
  Basis Update: $\Phi^{(k+1)} = snapshot\_pod(\{x_t\}_{t=0}^T)$\\
  $cost = cost + terminal\_cost({x^{k+1}_T}),$\\ \vspace{2pt}
  $\Delta cost(\alpha) = -\alpha \sum_{t=0}^{T-1} k_t' Q_{u_t}-\frac{\alpha^2}{2}\sum_{t=0}^{T-1}k_t'Q_{u_tu_t}k_t.$\\
  {\bf return} $u^{k+1}_{0:T-1}$, $cost$, $\Delta cost(\alpha)$
  \label{roILQR2}
\end{algorithm}
%

\begin{algorithm} 
% \footnotesize
  \caption{\strut Backward Pass}
  \CommentSty{/* start from the terminal time */}\\
  $t \gets T - 1$.\ \\
  Compute $J_{\bf x_T}$ and $J_{\bf x_T x_T}$ using boundary conditions.\\
  \While {$t >= 0$}{
  \CommentSty{/* Estimate the Jacobians using LLS-CD as shown in Section \ref{sec4}-1): */}\\
  $\bar{A}_t, \bar{B}_t \gets LLS-CD({ \bar{\alpha}_t},{\bar{u}_t}).$\\
  \CommentSty{/* Obtain the partials of the Q function as follows: */}
    \begin{equation*}
    \begin{split}
    Q_{\alpha_t} &= c_{\alpha_t}  + \bar{A}^T J_{\alpha_{t+1}},\\
    Q_{u_t} &= c_{u_t} + \bar{B}_t^T J_{\alpha_{t+1}},\\
    Q_{\alpha_t \alpha_t} &= c_{\alpha_t \alpha_t} + \bar{A}_t^T J_{\alpha_{t+1} \alpha_{t+1}} \bar{A}_t, \\
    Q_{u_t \alpha_t} &= c_{u_t \alpha_t} + \bar{B}_t^T (J_{\alpha_{t+1} \alpha_{t+1}} + \mu I_{l \times l}) \bar{A}_t, \\
    Q_{u_t u_t} &= c_{u_t u_t} + \bar{B}_t^T (J_{\alpha_{t+1} \alpha_{t+1}}+ \mu I_{l \times l}) \bar{B}_t.\\
    \end{split}
\end{equation*}
  \eIf{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t \alpha_t}.
    \end{split}
    \end{equation*}
    Decrease~$\mu$.
    }
    {
    Increase $\mu$.\\
    Restart backward pass for current time-step.
    }
  \CommentSty{/* Obtain the partials of the value function $J_t$ as follows: */}
  \begin{equation*}
      \begin{split}
          J_{\alpha_t} &= Q_{\alpha_t} + K_{t}' Q_{u_t u_t} k_t + K_t' Q_{u_t} + Q_{u_t \alpha_t}' k_t,\\
          J_{\alpha_t \alpha_t} &= Q_{\alpha_t \alpha_t} + K_t' Q_{u_t u_t} K_t + K_t' Q_{u_t \alpha_t} + Q_{u_t \alpha_t}' K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  {\bf return} $\{k_{0:T-1}, K_{0:T-1}\}$.
  \label{roILQR3}
\end{algorithm}


==> DDPGAlgorithm.tex <==
\subsection{\textbf{DDPG Algorithm}}
\label{sec:ddpg}
Deep Deterministic Policy Gradient (DDPG) is a policy-gradient based off-policy reinforcement learning algorithm that operates in continuous state and action spaces. It relies on two function approximation networks one each for the actor and the critic. The critic network estimates the $Q(s, a)$ value given the state and the action taken, while the actor network engenders a policy given the current state. Neural networks are employed to represent the networks. 

The off-policy characteristic of the algorithm employs a separate behavioral policy by introducing additive noise to the policy output obtained from the actor network. The critic network minimizes loss based on the temporal-difference (TD) error and the actor network uses the deterministic policy gradient theorem to update its policy gradient as shown below:

Critic update by minimizing the loss: 
\begin{equation*}
    L = \frac{1}{N} \Sigma_{i}(y_i - Q(s_i, a_i| \theta^{Q}))^2
\end{equation*}

Actor policy gradient update:
\begin{equation*}
    \nabla_{\theta^{\mu}} \approx \frac{1}{N} \Sigma_i \nabla_a Q(s,a|\theta^{Q})|_{s=s_i,a=\mu(s_i)} \nabla_{\theta^{\mu}} \mu(s|\theta^{\mu})|_{s_i}
\end{equation*}

The actor and the critic networks consist of two hidden layers with the first layer containing 400 ('{\it relu}' activated) units followed by the second layer containing 300 ('{\it relu}' activated) units. The output layer of the actor network has the number of ('tanh' activated) units equal to that of the number of actions in the action space.  

Target networks one each for the actor and the critic are employed for a gradual update of network parameters, thereby reducing the oscillations and a better training stability. The target networks are updated at $\tau = 0.001$. Experience replay is another technique that improves the stability of training by training the network with a batch of randomized data samples from its experience. We have used a batch size of 32 for the inverted pendulum and the cart pole examples, whereas it is 64 for the rest. Finally, the networks are compiled using Adams' optimizer with a learning rate of 0.001. 

To account for state-space exploration, the behavioral policy consists of an off-policy term arising from a random process. We obtain discrete samples from the Ornstein-Uhlenbeck (OU) process to generate noise as followed in the original DDPG method. The OU process has mean-reverting property and produces temporally correlated noise samples as follows:
\begin{equation*}
    dx_t = \Theta (\mu - x_t)dt + \sigma dW
\end{equation*}
where $\Theta$ indicates how fast the process reverts to mean, $\mu$ is the equilibrium or the mean value and $\sigma$ corresponds to the degree of volatility of the process. $\Theta$ is set to 0.15, $\mu$ to 0 and $\sigma$ is annealed from 0.35 to 0.05 over the training process. 

==> FAQ <==
***********************************************************************
Question 1:
Could  you please send the information regarding importing 
encapsulated postscript (*.eps) files (figures)  
into your *.tex and *.sty (asme.tex or asme.sty) provided. 
What should be the command I should add to the file and in which file, 
in *.sty or *.tex. Usually I add \input epsf in my *.tex file. 
Please let me know this way of importing the figure is acceptable.

Answer:
You may use the 'epsfig' package to incorporate an encapsulated postscript
figure into your document.  To include the package in LaTeX2e, use
"\usepackage{epsfig}" in the preamble of your document.  Use
"\epsfig{file=file.eps}" to incorporate the eps file in the figure environment.  
You may use width and/or height arguments to change the size
of the original figure, e.g. "\epsfig{file=file.eps,width=3in}."

If you are using LaTeX 2.09, use "\input{psfig}" in the preamble and use
"\psfig{figure=file.eps}" to include the eps file.  The height and width
arguments are the same.

Note: the argument for \epsfig{} and \psfig{} starts with 
"file=" and "figure=", respectively.

***********************************************************************
Question 2:
I am current preparing a paper to be submitted in an ASME conference.
There is a problem we are not able to solve. The problem is the
display of lower case Greek bold face font. 
Normally, the command 
\mbox{\boldmath${  ....  }$\unboldmath}
will do it. However, using the ASME template, this command seem not
function. I wonder if you had come across this problem before and
would share you experience with us.

Answer:
In LaTeX2e, use the \mathbf{} command
to make a bold math character.  
If that doesn't work, you will have to use an ams-LaTeX package.  

***********************************************************************
Question 3: 
How can I get bold italics?

Answer:
try \newcommand{\bAC}{\mbox{$\mathbf{AC}$}}
You could also try \textbf{\emph AC}

***********************************************************************
Question 4: 

I've been using your LaTeX2e asme2e.cls package to prepare a paper
for an upcoming conference, but have been having some trouble with the
fonts.  I was wondering if I might be able to ask you for a bit of
advice.

It seems as if none of the headings, titles, etc, are showing
up bold as they are supposed to.  When I run LaTeX, I get the
following...

{co.eng.caltech.edu:7} latex paper.tex
This is TeX, Version 3.1415 (C version 6.1)
(paper.tex
LaTeX2e <1994/12/01> patch level 1
(asme2e.cls
Document Class: asme2e 1997/04/10 v1.0 Standard LaTeX document class
(/ccovol/tex3/tex/latex/base/ifthen.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/times.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/mathptm.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/pifont.sty
No file Upzd.fd.

LaTeX Font Warning: Font shape `U/pzd/m/n ' undefined
(Font)              using `U/cmr/m/n' instead on input line 57.

No file Upsy.fd.

LaTeX Font Warning: Font shape `U/psy/m/n ' undefined
(Font)              using `U/cmr/m/n' instead on input line 58.




...and so on.

I noticed in the README2 file that there were some issues pertaining
to fonts.  Apparently I need to make sure that a new font package
(PSNFSS) is installed.  Does LaTeX's call to 

(/ccovol/tex3/tex/latex/packages/psnfss/times.sty)

imply that the sysadmins here have already done this?  In any case, I
tried to find the font packages at

http://tug2.cs.umb.edu/ctan/tex-archive/macros/latex/packages/psnfss/

but that address appears to have expired.  

If it is just a matter of installing these fonts, do you know of a new
address where I can get them?  And if it doesn't seem to be just a
problem of installing these fonts, do you have any ideas as to what
might be wrong?


Answer:
The problem is the  "pifont.sty" package uses the "Upzd.fd" and the "Upsy.fd"
font description files, which are missing in your installation of psnfss.  A
quick fix is to download the missing files from CTAN.  Point your browser to
http://www.ctan.org and click on the search link to search for the two files.
Download them to the same directory as your paper and rerun LaTeX2e.
You should ask your system administrators to install psnfss with the proper font
description files.



***********************************************************************
Question 5: 

How do you use .jgp and .png images as figures in LaTex when using PDF Texify?

Answer by Adam Pautsch at agpautsch@wisc.edu:
To include images, you must load the package "graphicx" in the preamble of 
the document. With the image file in the same folder as the .tex file, use 
the line "\includegraphics[keepaspectratio,width=3in]{filename.jgp}" to 
insert the image file. This may be included inside of a "figure" environment, 
which will allow for automatic captioning with the "\caption{}" command.

The images included in this manner will only appear when the "draft" option is
not used. When "draft" is used as an option, a box represnting an image with
the image's filename will appear in its place.

More information about handling images of different formats may be found at
     http://www.tex.ac.uk/cgi-bin/texfaq2html?label=dvipsgraphics
     http://www.tex.ac.uk/cgi-bin/texfaq2html?label=pdftexgraphics



==> Hybrid.tex <==
\subsubsection{Warm Starting(Model Based Approach)}
In  this  section, we derive a simple control scheme to control the inputs to each grid point in the material, so as to reach the desired phase distribution. In order to achieve this, we exploit the Allen-Cahn dynamics along with the assumptions of a periodic boundary condition to get a better initial estimate for the control scheme.

The Allen-Cahn equation has an interesting structure. Suppose we assume our system to be a single cell/pixel i.e. discretized as a 1X1 matrix. Owing to our assumption of a periodic boundary condition, the diffusion term effectively vanishes, i.e. $\nabla^2 \phi=0$. Thus, our dynamics reduce to 
\begin{equation}
    \frac{\partial \phi}{\partial t}=-M\frac{\partial f}{\partial \phi}=-M(4\phi^3+2T\phi+h)
\end{equation}
Thus, the simplified model reduces to a temporal differential equation instead of a complex spatio-temporal partial differential equation. This single pixel system is then fed to our iLQR-based control scheme, to generate a look-up table (of sorts) for a control trajectory from the given initial state $\phi_0$ to both stable final states $\phi_f=\pm 1$. 

The control trajectories thus obtained are mapped to any desired final state structure, and serve as an improved initial guess for the main algorithm, i.e. now the algorithm only has to optimize for the diffusion term.


\begin{figure}[!htb]
%\captionsetup{width=1\linewidth}



\begin{multicols}{2}
    %\hspace{3.2cm}
      \subfloat[]{\includegraphics[width=1\linewidth]{images/Hybrid/episodic_cost_training_original.png}}    
      \subfloat[]{\includegraphics[width=\linewidth]{images/Hybrid/episodic_cost_training_hyb.png}}
      %\subfloat[t=1.25s]{\includegraphics[width=0.8\linewidth]{images/50per/file49.png}}\\
      
         
\end{multicols}
%\begin{multicols}{6}
%\captionsetup{width=.75\textwidth}
    \caption{{Open loop training with starting guess initialised as (a)random control trajectory with zero mean, 
    (b)model based approach}} 
%\end{multicols}

\label{hyb_train}
\end{figure}

\begin{figure}
    %\centering
    \includegraphics[width=\linewidth]{images/Hybrid/trajComp.png}
    \caption{Comparing trajectories from model-based single-pixel method(no diffusion) with the optimized trajectory(with diffusion)}
    \label{fig:MSE_hyb}
\end{figure}



==> ILQR.tex <==
\subsection{Iterative Linear Quadratic Regulator Details}

% The Iterative LQR algorithm implemented here is a variation of the classical Differential Dynamic Programming(DDP) algorithm, wherein we constrain ourselves to just the first derivative of the dynamics.
% Let $U_t=\{u_i\}_{i=t}^{T-1}$. The cost-to-go is, thus, defined as
% \begin{equation*}
%     J_t(x,U_t)=\sum_{i=t}^{T-1} c(x_t, u_t)+\phi(x_T)
% \end{equation*}

% The value function at time \textit{t} is the cost-to-go given the minimising control sequence,
% \begin{equation*}
%     V_t(x) \equiv \min_{U_t} J_t(x, U_t).
% \end{equation*}

% Setting $V_T(x)=\phi(x_T)$, we can apply the Dynamic Programming Principle, which reduces the minimization over a sequence of controls to a sequence of minimizations over a single
% control, proceeding backwards in time:
% \begin{align*}
%     V_t(x)=\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))], \\
%     Q_t(x)=arg\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))]
% \end{align*}
% We define the action-value function as a function of perturbations around the pair $(x_t, u_t)$:
% \begin{align*}
%     Q_t(\delta x_t, \delta u_t)=c(x_t+\delta x_t, u_t+\delta u_t)-c(x_t, u_t) +\\
%     V_{t+1}(f(x_t+\delta x_t, u_t+\delta u_t))-V_{t+1}(f(x_t, u_t))
% \end{align*}
% and expand to the second order
% \begin{align}
%     Q_t(\delta x_t, \delta u_t) \approx \frac{1}{2}\begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}^T \begin{bmatrix}
%     0 &Q_x^T &Q_u^T\\
%     Q_x &Q_{xx} &Q_{xu}\\
%     Q_u &Q_{ux} &Q_{uu}
%     \end{bmatrix} \begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}
% \label{eq:ilqg_2nd_order}
% \end{align}
% The expansion coefficients can be written as 
% \begin{align}
%     &Q_x = c_x+f_{x}^T V'_{x} \label{eq:ilqg1} \\
%     &Q_u = c_u+f_{u}^T V'_{u} \label{eq:ilqg2} \\
%     &Q_{xx} = c_{xx}+f_{x}^T V'_{xx}f_{x} + V'_x \cdot f_{xx}  \label{eq:ilqg3} \\
%     &Q_{ux} = c_{ux}+f_{u}^T V'_{xx}f_{x}  + V'_x \cdot f_{ux} \label{eq:ilqg4} \\
%     &Q_{uu} = c_{uu}+f_{u}^T V'_{xx}f_{u}  + V'_x \cdot f_{uu}\label{eq:ilqg5} 
% \end{align}
% where $V' \equiv V_{t+1}$. The final terms in equations \ref{eq:ilqg3}, \ref{eq:ilqg4} and  \ref{eq:ilqg5} are ignored in ILQR. 

% Minimizing equation \ref{eq:ilqg_2nd_order} w.r.t. $\delta u$ gives
% \begin{equation}
%     \delta u^* = arg \min_{\delta u} Q_t(\delta x,\delta u) = -Q_{uu}^{-1}(Q_u+Q_{ux}\delta x)
% \end{equation}
% This gives an open-loop term $k=-Q_{uu}^{-1}Q_u$, along with the feedback gain term $K=-Q_{uu}^{-1}Q_{ux}$. Substituting the policy in equation \ref{eq:ilqg_2nd_order}, we have a quadratic model of the value function:
% \begin{align*}
%     &\Delta V(t) = -\frac{1}{2} Q_u Q_{uu}^{-1}Q_u \\ %\label{eq:ilqg1} \\
%     &V_x(t) = Q_x-Q_u Q_{uu}^{-1}Q_{ux} \\%\label{eq:ilqg2} \\
%     &V_{xx}(t) = Q_xx-Q_{xu} Q_{uu}^{-1}Q_{ux}  %\label{eq:ilqg3}
% \end{align*}

% The backward pass recursively computes the local quadratic models of $V(t)$ and ${k(t), K(t)}$. When the backward pass is completed, a forward pass of the algorithm then computes a new trajectory:
% \begin{align*}
%     &\hat{x}(0)=x(0) \\
%     &\hat{u}_t = u_t+k(t)+K(t)(\hat{x}(t)=x(t))\\
%     &\hat{x}(t+1)=f(\hat{x}(t), \hat{u}_t)
% \end{align*}


We present details of the D2C-ILQR algorithm in the following. The pseudo-code is given in Algorithm \ref{model_free_DDP_OL}. The `forward pass' and `backward pass' algorithms are summarized in Algorithms \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively. Algorithm \ref{model_free_DDP_feedback} presents the DDP feedback algorithm used to calculate the optimal feedback gain. 
\begin{algorithm}[!ht]
\footnotesize
  \caption{\strut Open-loop trajectory optimization via model-free ILQR}
  {\bf Input:} Initial State - ${\bf x_0}$, System parameters - $\mathcal{P}$\;
  $m \gets 1$. ~~\CommentSty{/* Initialize the iteration number $m$ to 1.*/}\\
  $forward\_pass\_flag$ = true. \\
  \CommentSty{/* Run until the difference in costs between subsequent iterations is less an $\epsilon$ fraction of the former cost.*/}\\
  \While {$m==1$ {\textnormal{or}} $({\text cost}(\mathbb{T}_{nom}^{m})/{\text cost}(\mathbb{T}_{nom}^{m-1})) < 1 + \epsilon$}{
  \CommentSty{/*Each iteration has a backward pass followed by a forward pass.*/}\\
  \{$k^{m}_{0:N-1}, K^{m}_{0:N-1}$\}, $backward\_pass\_success\_flag$ $=$ Backward Pass($\mathbb{T}_{nom}^{m}$, $\mathcal{P}$).\\
  \If{backward\_pass\_success\_flag == true}{
      $\mathbb{T}_{nom}^{m+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{m}$,$\{k^{m}_{0:N-1}, K^m_{0:N-1}\}$, $\mathcal{P}$).\\
      \While{forward\_pass\_flag == false}{
            $\mathbb{T}_{nom}^{m+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{m}$,$\{k^{m}_{0:N-1}, K^m_{0:N-1}\}$, $\mathcal{P}$).\\
            Reduce $\alpha$ from $\mathcal{P}$.    
        }
      }
  \Else{
        Increase $\mu$ from $\mathcal{P}$.~~\CommentSty{/* Regularization step */}\\
    }
      $m \leftarrow m + 1$. \\
  $\mathbb{T}^{*}_{nom} \gets \mathbb{T}^{m+1}_{nom}$.\\
  }
  
  {\bf return $\mathbb{T}^{*}_{nom}$}\\
  \label{model_free_DDP_OL}
\end{algorithm}

\begin{algorithm}[!htp]
\footnotesize
 \caption{\strut Forward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$ and system and cost parameters - $\mathcal{P}$.\
%   \CommentSty{/* Unpack the previous nominal trajectory.*/}\\
  $\{{\bar{x}_t^{prev}, \bar{u}_t^{prev}}\} \gets \mathbb{T}_{nom}^{k}$.\\
%   \CommentSty{/* Initialize time to 0.*/}\\
  $t \gets 0$.\\
  \While {$t < N$}{
    %\CommentSty{/*$\alpha$ is the line-search parameter.*/} \\
    \CommentSty{/*Simulate one step forward ($\alpha$ is the line-search parameter.)*/}
    \begin{equation*}
    \begin{split}
        {\bar{u}_{t}} &= {\bar{u}_t^{prev}} + \alpha k_t + K_{t} ({\bar{x}_t} - {\bar{x}_t^{prev}}),\\
        {\bar{x}_{t+1}} &= simulate\_forward\_step({\bar{x}_t}, {\bar{u}_t}).
        \end{split}
    \end{equation*}
    $t \leftarrow t + 1$. 
    }
  $\mathbb{T}_{nom}^{k+1}$ $\gets$ $\{{\bf \bar{x}_{0:N}}, {\bf \bar{u}_{0:N-1}}\}.$\\
  \If{$\mathbb{T}_{nom}^{k+1}$ to $\mathbb{T}_{nom}^{k}$ \textnormal{is acceptable}}{
    {\bf return} $\mathbb{T}_{nom}^{k+1}$, true.
  }
  \Else{
    {\bf return} $\mathbb{T}_{nom}^{k}$, false.
  }
  \label{model_free_DDP_OL_FP}
\end{algorithm}
%
\begin{algorithm}[!htp]
\footnotesize
  \caption{\strut Backward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Backward pass starts from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\
  \CommentSty{/*Keep a copy of previous policy gains.*/}\\
  $k\_old \gets k_{0:N}$ {and}  $K\_old \gets K_{0:N}$.\\
  
  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $f_{x_t}, f_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } $\{ k\_old, K\_old\}$, false.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $k\_new = k_{0:N-1},$\\
  $K\_new = K_{0:N-1}.$\\
  {\bf return} $\{k\_new, K\_new\}$, true.
  \label{model_free_DDP_OL_BP}
\end{algorithm}

\begin{algorithm} [!htp]
\footnotesize
  \caption{\strut DDP Feedback}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Start from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\

  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $h_{x_t}, h_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the Hessians from simulator rollouts as shown above:*/}\\
  $h_{x_tx_t}, h_{u_tx_t}, h_{u_tu_t} \gets model\_free\_hessian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t} + J_{x_{t+1}}^{\prime}h_{x_tx_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t} + J_{x_{t+1}}^{\prime}h_{u_tx_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t} + J_{x_{t+1}}^{\prime}h_{u_tu_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } error.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $K = K_{0:N-1}.$\\
  {\bf return} $\{K\}$, true.
  \label{model_free_DDP_feedback}
\end{algorithm}

% \subsection*{Estimation of Jacobians: Linear Least Squares by Central Difference (LLS-CD)}
% \label{sys_id_solve_supplementary}

% \textit{Note: The following is a more detailed discussion of section 4.1.1 in the main paper.}
% % We make a preliminary analysis on the number of evaluations required in the above algorithm. If the horizon is `$h$' and the number of iterations required to converge are `$n$', the algorithm requires us to estimate each of the $f_{\bf x_t}$ and $f_{\bf u_t}$ `$nh$' times. 


% % \begin{equation*}
% % \begin{split}
% %     &f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) + \begin{bmatrix} f_{\bf x_t}  f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T  \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix} +
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %     &f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) - \begin{bmatrix} f_{\bf x_t} f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix}+
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %   \end{split}
% % \end{equation*}
% Using Taylor's expansions of `$h$' (for generality, $h$ is the non-linear model of Section 2) about the nominal trajectory $(\bar{x}_t,  \bar{u}_t)$ on both the positive and the negative sides, we obtain the following central difference equation:\\
% $
%     h(\bar{x}_t + \delta x_t, \bar{u}_t + \delta u_t) - h(\bar{x}_t - \delta x_t, \bar{u}_t - \delta  u_t) =~2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \\ \delta {u_t} \end{bmatrix} + O(\| \delta {x_t}\|^2 + \| \delta {u_t}\|^2).
% $
% Multiplying by $\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix}$ on both sides to the above equation:
% \begin{equation*}
%     \begin{split}
%     \begin{bmatrix}h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) -  h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix} 
%      \times \begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} 
%     % &= 2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} \begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix}+ O(\| \delta {\bf x_t}\|^4 + \| \delta {\bf u_t}\|^4)\\
%      =2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix} \nonumber \\~~~~~~~~~~~~
%      + O(\| \delta {x_t}\|^3 + \| \delta {u_t}\|^3)
%      \end{split}
% \end{equation*}
% Assuming that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible (which will later be proved to be true by some assumptions), let us perform inversions on either sides of the above equation as follows:
% % \begin{equation*}
% %     \begin{split}
% %     &\begin{bmatrix}f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times\\
% %     &\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}^{-1} = \\&2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} +
% %      O(\| \delta {\bf x_t}\|^2 + \| \delta {\bf u_t}\|^2)
% %      \end{split}
% % \end{equation*}
% % $\implies$ 
% \begin{equation}
%     \begin{split}
%     \begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} 
%     &=\frac{1}{2}\begin{bmatrix} h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) - h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix}  \times\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T~ \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T ~\delta {u_t} \delta {u_t}^T \end{bmatrix}^{-1}\\ &~~~~~~~~~~~~~~~~~~+ O(\| \delta {x_t}\| + \| \delta {u_t}\|)
%      \label{eq : model_free_DDP_jacobian_raw1}
%      \end{split}
% \end{equation}
% Equation \eqref{eq : model_free_DDP_jacobian_raw1} solves for Jacobians, $h_{x_t}$ and $h_{u_t}$, simultaneously. It is noted that the above formulation requires only 2 evaluations of $h(.)$, given the nominal state and control $\-$ (${\bar{x}_t},{\bar{u}_t}$). The remaining terms (also, the error in the evaluation) are of the order that is linear in $\delta {x_t}$ and $\delta {u_t}$. The following extends equation \eqref{eq : model_free_DDP_jacobian_raw1} to be used in practical implementations (sampling).\\
% We are free to choose the distribution of $\delta {x_t}$ and $\delta {u_t}$. We assume both are i.i.d. Gaussian distributed random variables with zero mean and a standard deviation of $\sigma$.~This ensures that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible. Let `$n_s$' be the number of samples for each of the random variables, $\delta {x_t}$ and $\delta {u_t}$. Denote the random samples as $\delta {X_t} = \begin{bmatrix} \delta {x_t^1}& \delta {x_t^2}& \ldots &\delta {x_t^{n_s}}\end{bmatrix}$, $\delta {U_t} = \begin{bmatrix} \delta {u_t^1} &\delta {u_t^2}& \ldots& \delta {u_t^{n_s}}\end{bmatrix}$ and $\delta Y_t = \begin{bmatrix} \delta X_t & \delta U_t \end{bmatrix}$. Then $\begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix}$ is given by the following (via standard least squares):
% \begin{equation}
%     \begin{split}
%     &\begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} = H \delta Y_t^T (\delta Y_t\delta Y_t^T)^{-1} \\
%     &H = \begin{bmatrix} h({\bar{x}_t} + \delta {x_t^1}, {\bar{u}_t} + \delta {u_t^1}) - h({ \bar{x}_t} - \delta {x_t^1}, {\bar{u}_t} - \delta {u_t^1})\\ h({\bar{x}_t} + \delta {x_t^2}, {\bar{u}_t} + \delta {u_t^2}) - h({\bar{x}_t} - \delta {x_t^2}, {\bar{u}_t} - \delta {u_t^2}) \\ \vdots  \\h({\bar{x}_t} + \delta {x_t^{n_s}}, {\bar{u}_t} + \delta {u_t^{n_s}}) - h({\bar{x}_t} - \delta {x_t^{n_s}}, {\bar{u}_t} - \delta {u_t^{n_s}})\end{bmatrix}
%      \label{eq : model_free_DDP_jacobian1}
%      \end{split}
% \end{equation}
% Let us consider the terms in the matrix $\delta Y_t \delta Y_t^T=\begin{bmatrix}  \delta {X_t} \delta {X_t}^T & \delta {X_t} \delta {U_t}^T \\ \delta {U_t} \delta {X_t}^T  & \delta {U_t} \delta {U_t}^T \end{bmatrix}$.~$\delta {X_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T$. Similarly, $\delta {U_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T$, $\delta {U_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T$ and $\delta {X_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T$. From the definition of sample variance, for a large enough $n_s$, we can write the above matrix as 
% \begin{equation*}
% \begin{split}
%     \delta Y_t \delta Y_t^T &= \begin{bmatrix} \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T \\ \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T
%     \end{bmatrix}\\ &\approx \begin{bmatrix} \sigma^2(n_s - 1) {\text I_{n_x}} & {\text 0_{n_x \times n_u}} \\ 0_{n_u \times n_x} & \sigma^2 (n_s - 1) {\text I_{n_u}}\end{bmatrix} \\
%     &= \sigma^2 (n_s - 1){\text I}_{(n_x+n_u) \times (n_x+n_u)}
% \end{split}
% \end{equation*}

% \textit{Sample Complexity.} 
% Given that we have high enough number of samples $n_s$, typically `$O(n_x + n_u)$', the above approximation holds good. The reason is as follows. Note that the above least squares procedure converges when the matrix $\delta Y_t \delta Y_t^T$ converges to the identity matrix. This is entirely equivalent to estimation of the covariance of the  random vector $[\delta x_t \ \delta u_t]$ where $\delta x_t$, and $\delta u_t$ are Gaussian i.i.d. samples. Thus, it follows that the number of samples is $O(n_x+n_u)$, given $n_x+n_u$ is large enough \cite{HDP-book}. \\
% Note that if one were to use an FD procedure, the number of samples would be $O(n_x(n_x+n_u)) >> O(n_x+n_u)$. In fact, this behaviour is clearly apparent in our empirical results where FD is more efficient for low dimensional examples, while the LLS-CD procedure rapidly becomes much more efficient as the size of the examples increases. This has very important ramifications since the overwhelming bulk of the computations in our D2C implementation is in the estimation of these system dynamics. 

% \subsection*{Guarantees for ILQR}
% %\textcolor{red}{Can you add the iLQR/ DDP insight here?}\\
% As has been mentioned previously, iLQR is much more efficient than the related DDP procedure \cite{ddp} which requires the availability of the second order dynamics terms. Albeit this is known empirically \cite{ilqg2}, it is not clear as to why iLQR should provide a solution of the same quality as DDP? \\
% The reasoning for this as follows. 
% The DDP procedure is simply a sequential quadratic programming (SQP) procedure for the trajectory optimization problem, where the dynamics are the constraints in the optimization problem. In SQP, the Lagrangian, i.e., the cost function augmented with the constraints using the Lagrange multipliers, $\mathcal{L}(x,\lambda) = c(x) + \lambda h(x)$, where $c(x)$ is the cost function and $h(x) =0$ are the constraints, is expanded to second order about the current solution. In the context of trajectory optimization, this amounts to expanding the cost function to second order which also results in second order expansion of the dynamics. The only difference between DDP and iLQR is that, in iLQR, the second order expansion of the dynamics is neglected in the optimization problem.
% This is similar to idea of neglecting second order terms in Gauss-Newton's method (identical to iLQR) as compared to Newton's method (identical to DDP).
% Moreover, the guarantees for SQP, i.e., convergence to a stationary point of the augmented cost function still holds for iLQR. Therefore, it follows that we can expect iLQR to converge to a stationary point of the optimal control problem.\\
% Next, note that due to the Method of Characteristics development in the previous section, if the dynamics are affine in control and the cost is quadratic in control, it follows that satisfying the necessary conditions for optimality, which iLQR is guaranteed to do under mild conditions, one is assured of the global minimum to the problem. Then, a perturbation expansion of the characteristic equations about this optimal is guaranteed to give us at least a local solution to the HJB equation.% due to Proposition~\ref{T-PFC}.
% %Since the inversion of an identity matrix is trivial and always exists, the above matrix is invertible in equation \eqref{eq : model_free_DDP_jacobian1}. Thus, one can calculate $f_{\bf x}$ and $f_{\bf u}$ this way during the backward pass. For the sake of convenience in the later sections, let us refer to this method as `Linear Least Squares by Central Difference (LLS-CD)'. 
% %The entire algorithm to determine the optimal nominal trajectory in a model-free fashion is summarized together in Algorithm \ref{model_free_DDP_OL}. The detailed forward and backward pass functions are shown in Algorithm \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively in the supplementary material.

\subsection*{DDP Feedback Gain Calculation}
Once the optimal nominal trajectory is obtained with ILQR, one DDP back pass is conducted to find the linear optimal feedback gain as shown in Algorithm \ref{model_free_DDP_feedback}. Then the linear feedback is wrapped around the nominal control sequence ($u_t = \bar{u}_t + K_t\delta x_t$),where $\delta x_t$ is the state deviation from the nominal state $\bar{x}_t$.

% \sr
% \begin{align}
% z_i &= \begin{bmatrix} \delta {x}^T & \delta {u}^T \end{bmatrix} \begin{bmatrix} h_{xx}^{(i)}  & h_{xu}^{(i)}  \\ h_{ux}^{(i)}  & h_{uu}^{(i)}  \end{bmatrix} \begin{bmatrix}  \delta {x} \\ \delta {u} \end{bmatrix} \nonumber \\  \nonumber
% &= \sum_{j=1}^{n_s} \sum_{k=1}^{n_s} \dfrac{\partial^2 h_i}{\partial x_j \partial x_k} \delta x_j \delta x_k + 2 \sum_{p=1}^{n_u} \sum_{q=1}^{n_s} \dfrac{\partial^2 h_i}{\partial u_p \partial x_q} \delta u_p \delta x_q + \sum_{d=1}^{n_u} \sum_{h=1}^{n_u} \dfrac{\partial^2 h_i}{\partial u_d \partial u_h} \delta u_d \delta u_h \\ \nonumber
% &= \underbrace{\begin{bmatrix} \delta {x_1}^2 & \delta {x_1} \delta {x_2} & \cdots & \delta {x_1} \delta {u_{n_u}} & \delta {x_2}^2 & \delta {x_2} \delta {x_3} & \cdots& \delta {u^2_{n_u}}\end{bmatrix}}_{\delta {XU}}  \underbrace{\begin{bmatrix} \dfrac{\partial^2 h_i}{\partial x_1^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial x_2} \\ \vdots \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial u_{n_u}} \\ \\ \dfrac{\partial^2 h_i}{\partial x_2^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_2 \partial x_3} \\ \vdots \\ \dfrac{\partial^2 h_i}{\partial {u^2_{n_u}}}\end{bmatrix}}_{H_i},\\
% \end{align}
% % \begin{bmatrix} \delta {x_1} & \delta {x_2} & \cdots & \delta {x_{n_s}} & \delta {u_1} & \delta {u_2} & \cdots & \delta {u_{n_u}} \end{bmatrix} 

% where $h_{xx}^{(i)} = \left.\dfrac{\partial^2 h_i}{\partial x^2}\right|_{x=t}$, $z_i$ is the $i^{th}$ element of vector $z_t$ and $h_i$ is the $i^{th}$ element of the dynamics vector $h(x_t, u_t)$. Multiplying on both sides by $\delta XU^T$ and apply standard Least Square method:
% $H_i = (\delta XU^T \delta XU)^{-1} \delta XU^T Z_i$. Then repeat for $i=1,2,...,n_s$ to get the estimation for the Hessian tensor.

==> Introduction_revised.tex <==
\section{Introduction}

The modeling and control of infinite-dimensional partial differential equations has long been a topic of avid interest, extending into various different fields ranging from fluid flows \cite{lellouche}, protein folding and enzyme kinematics \cite{proteinfold}, to microstructure dynamics \cite{Boe2002}\cite{Rui2011}. Such problems are usually solved by employing numerical methods, discretizing the state space through finite-element methods and controlling the resulting very high-dimensional system of differential equations. The need for dimensionality reduction in such systems paved the way for Model Order Reduction (MOR) techniques, accomplished in a data-driven manner, using techniques such as DMD \cite{dmd1}\cite{dmd2}, neural networks \cite{nn1}\cite{nn2}\cite{autoenc}, nonlinear auto-regressive algorithms\cite{nara1}, and sparse regression\cite{sparse1}. Perhaps the most widely used approach is the so-called Proper Orthogonal Decomposition (POD) Method of Snapshots that finds a reduced basis for the approximation of the nonlinear PDE using snapshots from a simulation of the same\cite{sirovich1987turbulence}. 


% \textcolor{red}{the original POD paper is not by Lall, its from Fluids, by Sirovich, please reference that paper.} }
% \textcolor{blue}{%Despite a lot of progress in the field, the control of nonlinear systems still remains a challenging problem. Methods for nonlinear control design, such as sliding mode control \cite{smcreview}\cite{nonlinearsmc}, backstepping and Lyapunov function analysis \cite{krstic1995nonlinear}\cite{vaidyanathan2020backstepping} have been developed and have been shown to work with a wide range of low-dimensional applications.}
In previous work \cite{wang2021search}\cite{yu2019decoupled}, the authors proposed a data-based algorithm for optimal nonlinear control, which identifies successive linear time-varying (LTV) models combined with the so-called Iterative Linear Quadratic Regulator (ILQR) approach to yield a globally optimum local feedback law. The ILQR algorithm \cite{li2004iterative} is a sequential quadratic programming (SQP) approach, typically used to solve nonlinear programming problems, for the solution of optimal control problems, and under relatively mild conditions can be shown to converge to the global minimum of the optimal control problem \cite{wang2021search}. The ILQR is a versatile approach and has been successfully applied to a wide range of relatively low-dimensional robotic applications \cite{ilqr2}\cite{ilqr3}. %with several extensions to the algorithm, such as the iterative LQG \cite{todorov2005generalized} further diversifying the applications of the original algorithm. 
%The complexity of solving nonlinear control problems increases exponentially when tacked on with the Curse-of-Dimensionality, resulting from solving for very high-dimensional problems. 
Unfortunately, none of these extensions address the intractability of the ILQR algorithm when dealing with high-dimensional systems, in particular PDEs that require the identification of very high-dimensional LTV models and leads to intractability of the critical backward pass Ricatti recursion in the algorithm. Hence, the optimal control of nonlinear PDEs still remains a major challenge.

\begin{figure}
    \centering
    % \includegraphics[width=0.8\linewidth]{images/temporal_disc.png}
\begin{multicols}{4}
      \subfloat[Initial State]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj11.png}}
      \subfloat[Int. I]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj12.png}}
      \subfloat[Int. II]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj13.png}}
      \subfloat[Final State]{\includegraphics[width=\linewidth]{images/roilqr plots/Trajm14.png}}
      
      
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}
\begin{multicols}{4}
   
       
      \subfloat[1st mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis11.png}}
      \subfloat[2nd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis12.png}}
      \subfloat[3rd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis13.png}}
      \subfloat[4th mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis14.png}}
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}

\begin{multicols}{4}
   
      \subfloat[Initial State]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj201.png}}
      \subfloat[Int. I]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj202.png}}
      \subfloat[Int.  II]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj203.png}}
      \subfloat[Final State]{\includegraphics[width=\linewidth]{images/roilqr plots/Trajm204.png}}
      
      
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}

\begin{multicols}{4}
   
       
      \subfloat[1st mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis201.png}}
      \subfloat[2nd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis202.png}}
      \subfloat[3rd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis203.png}}
      \subfloat[4th mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis204.png}}
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}


    %\caption{Comparing control cost at different time-discretizations}
    \caption{\small The initial trajectory (a)-(d) differs significantly from the final trajectory optimized by ILQR (i)-(l). Thus, the set of basis eigenfunctions for the initial trajectory (e)-(h) will only be valid locally, and differ significantly from the reduced order subspace that the optimal trajectory lies on (m)-(p). Hence, it is key to update the reduced-order basis with each successive iteration of the algorithm.}
    \label{fig:up_top}

\end{figure}

% \textcolor{blue}{Add papers on reduced order MBRL. Typically, the algorithms are split between a 'reduce-then-optimize', or an 'optimize-then-reduce' approach. These approaches suffer from model bias arising from differing basis as the optimization proceeds, leading to a need for shifting the RO basis as we iterate locally.}
The field of PDE control has a rich history, for instance, see Kunisch \cite{KunischOCPDE}, %\cite{KunischSLPDE},
 Volkwein \cite{volkweinPhaseField}, %\cite{VolkweinParabolicADR},
%Krstic \cite{smyshlyaev2010adaptive}, Alla \cite{allaSLPDE} 
and Falcone \cite{allafalconeadaptive}. %This foundational work was further built upon for application to nonlinear PDE control \cite{Breiten}\cite{bennerOCPDE}\cite{VolkweinFeedbackController}\cite{volkweinNonlinearRDE}\cite{krstic2008backstepping}.
% Further work by Luo et al \cite{cybernetics} suggests using a Karhunen-Loève decomposition followed by singular perturbation for model order reduction, and a neural network (NN)-based approach to solve the HJB-like equation in order to compute an approximate optimal control for nonlinear one-dimensional PDEs. 
More recently, there is a shift towards the application of reinforcement learning techniques for the control of such distributed parameter systems \cite{tnnls_pde_2}, in conjunction with model reduction approaches such as the Karhunen-Loève decomposition \cite{cybernetics}. These techniques are broadly classified into a ``reduce-then-control" (RTC) approach \cite{rtc_1,rtc_2}, and a ``control-then-reduce" (CTR) approach \cite{ctr_1}. However, in general, the CTR approach is infeasible, due to the intractability of finding the control for the full-order models in very high-dimensional problems (Curse of Dimensionality).
Recent work from Kramer et al \cite{Kramer-ILQR} have suggested using a linear time invariant (LTI) model reduction technique called Balanced Truncation \cite{tacBT} %\cite{BTLQG}
 to obtain a reduced basis on which to project the nonlinear PDEs to obtain a reduced order nonlinear model, the optimal control for which is then accomplished using the ILQR algorithm.  However, in general, the reduced basis modes can be quite different around the optimal trajectory when compared to an initial trajectory, and an approximation using the latter’s reduced basis can lead to unacceptable performance \cite{ravindran2002}\cite{kunisch2008}. %(also see Fig. 1). 
 Therefore, the reduced basis needs to be adaptively changed as the optimization proceeds \cite{kunisch2008}\cite{pod_volkwein}. Moreover, for nonlinear PDEs, the model reduction still results in a lower order nonlinear model, whose optimal control is itself challenging, and in general, intractable. %Further, it is not clear how one improves on the reduced order model to converge to the optimal trajectory. 
\textit{In this regard, the simple yet fundamental observation we make is that since the Proper Orthogonal Decomposition (POD) basis is local, an LTV model suffices to approximate the local behavior of the nonlinear PDE rather than a reduced nonlinear model.} %This enables us to use a reduced order version of the ILQR approach where we recursively change the reduced basis for successive trajectories using the method of snapshots and obtain reduced order LTV systems around the current estimate. This allows to recursively use reduced order LTV control techniques to solve for the optimal nonlinear control in a highly efficient fashion.} }\\

Thus, in this paper, we introduce a reduced order model based RL approach, which modifies the existing Iterative Linear Quadratic Regulator (ILQR) technique to an "iterative-reduce-then-control" (IRTC) method for the optimal control of nonlinear PDEs. The ILQR approach is implemented in a data-based/ MBRL fashion, wherein we use rollouts by querying the `black-box' computational model. It %Iterative Linear Quadratic Regulator (RO-ILQR) approach for the optimal control of nonlinear PDEs. The ILQR approach 
iteratively linearizes the dynamics and quadratizes the cost function around the current estimate of the optimal trajectory, solves a time varying LQR problem to find an improved control sequence, and repeats the process till convergence. In this paper, we use the POD Method of snapshots \cite{sirovich1987turbulence} to find a reduced order LTV approximation of the PDE around the current trajectory, solve a reduced order LQR problem to find an improved trajectory along with an updated POD basis, and iterate till convergence, thereby drastically reducing the computational burden of the ILQR approach when applied to PDEs. The proposed approach is tested on the viscous Burger's equation and on two phase field models for reaction-diffusion equations describing microstructure evolution in multi-phase materials and is shown to converge to the global optimum that would result without the model reduction. This paper is an extension %of our previous conference 
to the work done in \cite{roilqr}: it introduces a convergence analysis for the quality of the solution provided by the reduced order approach and gives more extensive computational results.
%\noindent The contributions of the paper are as follows:
%\begin{itemize}
    % \item We show how to model the dynamics of a multi-phase micro-structure and unveil its underlying structure.
 %   \item We propose a reduced order ILQR (RO-ILQR) algorithm for the control of systems that are governed by complex, nonlinear PDEs, using the POD method of snapshots to find local reduced order LTV approximations of the nonlinear PDE around a current trajectory.
    
  %  \item We compare the proposed RO-ILQR approach to the full-order ILQR algorithm, and show that the reduced order approach significantly reduces the computational burden, albeit with a small loss in optimal performance owing to the model reduction, when operating on high-dimensional PDEs.  
   
%\end{itemize}



%\section{Related Work}
The rest of the paper is organized as follows: In Section \ref{sec2}, we introduce the PDE nonlinear optimal control problem. We discuss the issues related to control of high-dimensional PDEs, and suggest ways to navigate around them in Section \ref{sec3}. In Section \ref{sec4}, we briefly introduce the iLQR algorithm, followed by the proposed approach. In Section \ref{analysis}, we show a mathematical analysis for the convergence guarantees of the proposed approach.
Section \ref{sec5}
illustrates the application of the proposed approach through custom-defined test problems of varying dimensions, along with repeatability, followed by the benchmarking of the approach with the standard ILQR.

\vspace{-0.15cm}

==> PerturbationModel.tex <==

From Eq. \ref{rodyn}, we know the reduced-order dynamics are:
\begin{equation*}
    \alpha_{t+1}=\Phi^T f(\Phi \alpha_t)+\Phi^Tg(\Phi \alpha_t)u_t
\end{equation*}

Taking perturbations $\alpha_t= \bar{\alpha}_t+\delta \alpha_t$, and $u_t= \bar{u}_t+\delta u_t$, we linearize the system about the trajectory, to get a linear time-varying approximation of the non-linear dynamics about the trajectory. \textcolor{red}{Is the equation below correct? This is the critical part of the work, please describe it carefully!}

\begin{align*}
    \delta \alpha_{t+1}&=\Phi^T(\frac{\partial f}{\partial \Phi \alpha_t}+\frac{\partial g}{\partial \Phi \alpha_t}u_t)\Phi \delta \alpha_t + \Phi^T g(\Phi \alpha_t)\delta u_t\\
    &=\Phi^T(\frac{\partial f}{\partial x_t}+\frac{\partial g}{\partial x_t}u_t)\Phi \delta \alpha_t + \Phi^T g(x_t)\delta u_t\\
    &= \bar{A}_t\delta \alpha_t + \bar{B}_t\delta u_t
\end{align*}

where $\bar{A}_t$ and $\bar{B}_t$ are the unknown matrices of dimensions $(l\times l)$ and $(l\times p)$ respectively. These can be identified using the Linear Least-Squares approach. \textcolor{red}{Describe!}

Thus, the system identification problem reduces from $O(N+p)$ to $O(l+p)$, where $l\ll n_x$. \\

The new parameters being identified assume some loss in information of the dynamics due to projection on a reduced order basis. But from perturbation experiments, we observe that the reduced-order LTV system can almost fully track the same level of performance in capturing the dynamics as the full-order LTV system as seen in Fig. \ref{ltv_podvsfo}, despite a significantly cheaper computation cost.  

\begin{figure}[!htpb]

    \includegraphics[width=\linewidth]{images/roilqr plots/sys_id_10pc_comp.png}\\
    \includegraphics[width=\linewidth]{images/roilqr plots/sys_id_30pc_comp.png}
% \begin{multicols}{2}
%     %\hspace{1.4cm} 
%       \subfloat[Initial state]{\includegraphics[width=\linewidth]{images/roilqr plots/sys_id_10pc_comp.png}}    
%       \subfloat[Initial state]{\includegraphics[width=\linewidth]{images/roilqr plots/sys_id_30pc_comp.png}}
      
% \end{multicols}
\caption{{Relative performance of the Full-order vs Reduced-order LTV systems identified wrt the ground truth. The trajectory is appended with a Gaussian noise of std 10\% and 30\% of the max control input.}}
\label{ltv_podvsfo}
\end{figure}

==> Replanning.tex <==
\subsubsection{Model Predictive Control}

To reduce the variance of the policy in high noise regimes, we advocate the use of a rapid open loop solver along with replanning at every step, i.e. a \textbf{Model-Predictive Control} approach, to solve the RL problem, since MPC should be able to recover the global optimality for these problems \cite{mohamed2020near}.

 The recursive MPC algorithm implemented, which uses a fast and reliable local-planner, is summarised in Algorithm \ref{alg3}, and Figure \ref{fig:replan_error} compares the robustness to noise between the stochastic policy obtained from the recursive MPC with the decoupled closed-loop feedback policy at varying noise regimes.
 
 \begin{algorithm}
    \caption{Recursive MPC Algorithm}
    \label{alg3}
   {\bf 1)}  \textit{Given:} Initial state $x_0$, time horizon $T$, cost $c(x,u)=l(x)+\frac{1}{2}ru^2$, and terminal cost $c_T(x)$.\\
  {\bf 2)} Set $H=T$, $x_i = x_0$.\\
%   {\bf 3)} Solve the Riccati equations for each step along the nominal trajectory for feedback gain $\{ K_t \}_{t = 0}^{T-1}$.\\
%   {\bf 4)} Apply the closed-loop control policy,
  
\While{$H >0$}{
  \begin{enumerate}
        \item Solve the open-loop(deterministic) optimal control problem for initial state $x_i$ and horizon $H$. Let the optimal sequence be $U^*=\{u_0, u_1,...u_{H-1}\}$.
        \item Apply the first control $u_0$ to the stochastic system,\\
        and observe the next state $x_n$.
        \item Set $H=H-1, x_i = x_n$
\end{enumerate}
}
\end{algorithm}

 We observe that re-planning at every time-step easily recovers the optimality over all noise-regimes. Also, owing to the rapid convergence of the open-loop solvers for the material micro-structures, the extra computation cost which arises due to the repeated iterations of the open-loop solver, is not very significant, and can be reduced even further by integrating the MPC approach with a warm-start optimization (Figure \ref{fig:rep_train_times}).
 


\begin{figure}[!htb]
%\captionsetup{width=1\linewidth}



\begin{multicols}{2}
    %\hspace{3.2cm}
      \subfloat[]{\includegraphics[width=1\linewidth]{images/Replan_comp_plots/comp_time_replan.png}}    
      \subfloat[]{\includegraphics[width=\linewidth]{images/Replan_comp_plots/cml_comp_time_replan.png}}
      %\subfloat[t=1.25s]{\includegraphics[width=0.8\linewidth]{images/50per/file49.png}}\\
      
         
\end{multicols}
%\begin{multicols}{6}
%\captionsetup{width=.75\textwidth}
    \caption{{Computation times for re-planning with the recursive MPC approach}} 
%\end{multicols}

\label{fig:rep_train_times}
\end{figure}

==> Reviews_CDC2020.tex <==
% Reviewer 2 of CDC 2020 submission 1279

% Comments to the author
% ======================

% In the submission „Optimal Control of Material
% Micro-Structures” the authors consider a so called
% Allen-Cahn equation, which is an diffusion equation for the
% mixture of two phases, driven by nonlinear indomain
% actuation. For 100% concentration of one phase, the state
% is equal -1, for 100 % concentration of the other phase,
% the state is equal +1. For the actuation both the
% temperature and an external force field can be assigned
% arbitrarily for any time and location. A “model based
% control” (which is only the steady-state control input) is
% compared with the proposed “decoupled data based control
% (D2C)”. The latter, is based on an optimization of an
% feedforward trajectory and an feedback. 

% I cannot recommend acceptance, for the following reasons:
% The distributed character of the plant is not considered.
% For the “model based control”, the diffusion is ignored and
% only a constant control input is considered. For the “D2C”
% approach, the dynamics are approximated with a lumped,
% time-discrete system that results from an identification
% and is not deduced by the distributed system model. In
% general, the aspect, that the state is bounded on [-1, +1],
% is ignored in the design. 


% Reviewer 3 of CDC 2020 submission 1279

% Comments to the author
% ======================

% The paper addresses an optimal control problem for material
% micro-structures. The paper is rather unusual for classical
% control theory, since strongly relying on physical
% consideration of so-called Phase Fields and associated
% material properties. Still the paper might be interesting
% for CDC auditorium if properly written. Several remarks and
% comments are given below.

% -	“for the control of these systems” might be
% confusing, since not fully clear whether production or
% exploitation processes of material micro-structures are
% meant here. The Authors are welcome to put more
% straightforward description of problem statement within the
% Introduction part.

% -	“Number of new algorithms” you are referring to,
% i.e. [14]-[16] are all arXiv records. Please elaborate more
% on presenting state of the art and including also adequate
% available published literature.

% -	Better distinguish your recent contribution from
% the previous work [18].


% -	By your assumption of \phi, after eq. (1), it has
% only two binary states. This provides the system with a
% kind of hybrid, correspondingly switching dynamics. How do
% you deal with this, correspondingly capture the transitions
% between such two-state (phases) of the system?


% -	In view of that T is one of your control variables,
% temperature, an exposition in Sec. I.A-B with discrete
% values, like T={-2,-1,0,1,2} is less clear, or at  least
% not clear from reading.

% -	In Section IV, the step from the nonlinear affine
% in control dynamics (10) to the linearized state-space
% notation is not well described. In total, the Section IV,
% which is more relevant from the control viewpoint, is not
% fluently readable.

% -	In total, the Algorithm 1 appears as an iterative
% procedure of state discretization, obtaining set of local
% LTV models, and designing standard LQR regulator by Riccati
% approach. What is here special or new as for control
% design?

% -	The analysis of resulted control system dynamics
% and stability related issues are missing. 

% -	The overall presentation of the Section V can be
% improved, for making evaluation, correspondingly, test
% scenarios more comprehensible for readers.



% Reviewer 4 of CDC 2020 submission 1279

% Comments to the author
% ======================

% Content
% The authors apply the decoupled data based control approach
% to control the distributed parameter system describing
% material micro-structures. The multi-phase microstructure
% is described the Allen-Cahn equation. The control, is
% basically the offline computed feed-forward control which
% is constant over time.

% The paper is well written and deals with an interesting
% topic. 

% Major remarks:

% The authors should comment more detailed on the possibility
% of reaching only local minima. 

% %% COVERED IN AISTATS PAPER

% Why are the input restricted to be constant? 

% The linear time-varying system identification section
% should be detailed further. A comparison to other
% techniques would be interesting.

% Minor remarks:
% It would be interesting to know, which kind of application
% the authors have in mind, as it is difficult to generate
% two inputs over a plane, e.g. only a temperature
% distribution might be achieves with local heating elements.

% The results of the baseline controller in comparison to the
% optimized control results would be interesting.



==> Simulations.tex <==
\section{Empirical Results}\label{sec5}

% % In this section, we show the performance of the RO-ILQR approach on several nonlinear PDEs and compare its performance with the standard ILQR approach.

\subsection{Optimal Control Problems Studied}
\label{applications}

This section introduces the PDEs used for comparing the reduced order ILQR with the standard ILQR approach implemented on a full-order, high DOF system.

% The PDEs were spatio-temporally discretized using a Central-Difference scheme.
% \textcolor{red}{Get the equations out of inline below.}
\subsubsection{1D Viscous Burger's Equation}
Consider the viscous Burger's Equation:
\begin{equation*}
    \frac{\partial u}{\partial t}+u \frac{\partial u}{\partial x}=\nu \frac{\partial^2 u}{\partial x^2},
\end{equation*}
with external control inputs on the boundaries corresponding to blowing/suction such that $u(0,t)=U_1(t)$; $u(L,t)=U_2(t)$.


\subsubsection{Material Microstructure evolution - Allen-Cahn and Cahn-Hilliard Equation}
The evolution of material micro-structures can be represented by two types of partial differential equations, i.e., the Allen-Cahn (A-C) equation \cite{ALLEN19791085} representing the evolution of a  non-conserved quantity, and the Cahn-Hilliard (C-H) equation \cite{Cahn1958} representing the evolution of a conserved quantity. The Allen-Cahn equation has the general form %$\frac{\partial \phi}{\partial t}= -M(\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi),$ %\\
\begin{align}
    \frac{\partial \phi}{\partial t}= -M(\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi), %\label{eq:Dyn_main}
\end{align}
while the Cahn-Hilliard equation has the form %$\frac{\partial \phi}{\partial t}= \nabla \cdot M \nabla (\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi)$,
\begin{align}
    \frac{\partial \phi}{\partial t}= \nabla \cdot M \nabla (\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi), %\label{eq:Dyn_main}
\end{align}
where $\phi=\phi(x,t)$ is called the order parameter. In Controls parlance, $\phi$ is the state of the system, and is infinite dimensional. It reflects the component proportion of each phase of material system. For a two-phase system studied in this work, $\phi$ = -1 represents one pure phase and $\phi$ = 1 represent the other, while $\phi$ $\in$ (-1, 1) stands for a combination state of both phases on the boundary interface between two pure phases; \textit{M} is a parameter related to the mobility of material, which is assumed \textit{constant} in this study; \textit{F} is an energy function with a nonlinear dependence on $\phi$; $\gamma$ is a gradient coefficient controlling the diffusion level or thickness of the boundary interface.

In this study, we adopt the following general form of energy density function %\textcolor{blue}{Please give reference}:
\begin{align}
    F(\phi;T,h) = \phi^{4}+T\phi^{2}+h\phi . \,%\label{eq:D_well} 
\end{align}
Here, the parameters \textit{T} and \textit{h} are not governed by the A-C and C-H equations. Instead, they may be externally set to any value and may be spatially as well as temporally varying. 


% \vspace{-0.3cm}
% \input{pde_introduction.tex}
% \vspace{-0.2cm}
\subsection{Structure and Task}
We simulated the dynamics in Python, through calling an explicit, second-order solver subroutine in FORTRAN. The system and its tasks are defined as follows: 
\begin{figure}[!htpb]
\vspace{-0.5cm}
\begin{multicols}{3}
    %\hspace{1.4cm} 
      \subfloat[Initial state]{\includegraphics[width=\linewidth]{images/Initial_state.PNG}}    
    %   \subfloat[Goal state-I]{\includegraphics[width=\linewidth]{images/Final_state.PNG}}
      \subfloat[Goal state-I]{\includegraphics[width=1.1\linewidth]{images/roilqr plots/CH_GS.png}}
      \subfloat[Goal state-II]{\includegraphics[width=\linewidth]{images/Final_state_4.PNG}}

\end{multicols}
% \begin{multicols}{2}
%     %\hspace{1.4cm} 
          
%       \subfloat[Goal state-II]{\includegraphics[width=0.5\linewidth]{images/Final_state_2.PNG}}
%       \subfloat[Goal state-III]{\includegraphics[width=0.5\linewidth]{images/Final_state_4.PNG}}

% \end{multicols}
\caption{{Model simulated in Python}}
% \vspace{-0.4cm}
\label{figinit}
\end{figure}



\paragraph{Material Micro-structure}
The material model simulated consists of a 2-dimensional grid of dimensions $20 \times 20$ and $50 \times 50$ i.e.,  400 and 2500 fully observable states respectively. The order parameter at each of the grid point can be varied in the range $[-1, 1]$. Furthermore, the model is solved using an explicit, second order, central-difference based scheme. The control inputs $(T, h)$ are actuated such that all the grid-points with target order-parameter as +1 are fed the same control inputs, while a different set of $(T, h)$ is fed to those with the target as -1.\\
The control task is to influence the material dynamics to converge at a 
custom phase-distribution, with 2500 state variables and 4 control channels.

The initial and the desired final state of the model are shown in Fig. \ref{figinit}. 

\paragraph{1D Viscous Burgers Equation}
The Burgers equation PDE is modeled as a 1-dimensional grid discretized using a Finite Difference scheme, with 100 equally-spaced grid points serving as 100 fully-observable states. The model is solved using an explicit, second order, central-difference based scheme as well. The system has two suction/blowing control inputs at the boundaries, thus there being two control variables.

Given an initial velocity profile $u(x,0) = sin(\pi x)$ for $x\in [-1,1]$, the control task is to reach the goal state $u(x,T)=-0.5$ (constant velocity profile).

\begin{remark}
    Note that, for the purpose of the study, the dimensionality of the systems considered were kept within $O(10^3)$, which is smaller than realistic grid scales. This is done to facilitate a comparison with the full-order solution since the standard, full-order ILQR becomes intractable as we scale the dimensionality of the problem. Thus, in order to establish a benchmark with the ground truth (here, the solution from the ILQR), the experiments were restricted to dimensions where the full-order approach can still yield a feasible solution.
\end{remark}
% as given in Fig.~\ref{bginitfin} (a) and (b). 
% \begin{figure}[!htp]
% %\captionsetup{width=1\linewidth}



% \begin{multicols}{2}
%     % \hspace{3.2cm}
%       \subfloat[Initial Velocity Profile]{\includegraphics[width=\linewidth]{images/Burgers/burgers_init.png}}    
%       \subfloat[Target Velocity Profile]{\includegraphics[width=\linewidth]{images/Burgers/burgers_goal.png}}
      
      
% \end{multicols}

% %\begin{multicols}{6}
% %\captionsetup{width=.75\textwidth}
%     \caption{{Initial and goal state for Burgers Equation modeled in Python}} 
% %\end{multicols}

% \label{bginitfin}
% \end{figure}
% The model starts at an initial configuration of all states at $\phi=-1$. The final state should converge to alternating bands of $\phi=0$ (red) and $\phi=1$ (blue), with each band containing 2 columns of grid-points. 


% \subsection{Algorithms Tested}
% % \input{Hybrid.tex}
% %\subsubsection{Model Based Control}
% %% REMOVE THIS LINE FOR JOURNAL
% \paragraph{ILQR} One paragraph introduction to ILQR, add Algorithm 

%% REMOVE THIS LINE FOR JOURNAL
%\input{MaterialControl.tex}
%\input{DDPGAlgorithm.tex}

\subsection{Training and Testing}
\subsubsection{Open-loop trajectory convergence}

The open-loop training plots in Fig.~\ref{d2c_2_training_testing} show the cost curve during training. After the cost curves converge, we get the optimal control sequence that could drive the systems to accomplish their tasks. %The model position at the end of the horizon is shown in Fig.\ref{figfinal}.
The training parameters and outcomes are summarized in (Tables \ref{d2c_comparison_table1}, \ref{params_comp}).
The optimal trajectories obtained for the Allen-Cahn and Burgers PDE are shown in Fig.~\ref{AC_traj} and ~\ref{bg_traj} respectively.

\begin{figure*}[!htpb]
\centering
% \begin{multicols}{3}
   
%       \subfloat[DDPG Convergence]{\includegraphics[width=1\linewidth]{images/DDPG_Plots/ddpg_banded_h_100.png}}    
%       \subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/Training/Banded_episodic_cost_OL_training.png}}
%       \subfloat[ILQR-based D2C Convergence]{\includegraphics[width=1\linewidth]{images/Training/Banded_D2C_2.png}}\\
      
      
% \end{multicols}
% \begin{multicols}{3}
   
%       \subfloat[DDPG Convergence]{\includegraphics[width=1\linewidth]{images/DDPG_Plots/ddpg_checkerboard_h_10_10000r.png}}    
%       \subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/Training/episodic_cost_OL_training_20x20.png}}
%       %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
%       \subfloat[ILQR-based D2C Convergence]{\includegraphics[width=1\linewidth]{images/Training/Figure_20X20.png}}\\
      
      
% \end{multicols}
% \centering
\begin{multicols}{3}
\ 
      \subfloat[Allen-Cahn Convergence\\(GS-II)]{\includegraphics[width=1\linewidth]{images/roilqr plots/AC50x50.png}}
      \subfloat[Cahn-Hilliard Convergence\\(GS-I)]{\includegraphics[width=1\linewidth]{images/roilqr plots/CH_conv.png}}
      %/DDPG_Plots/ddpg_checkerboard_h_10_10000r.png}}
      \subfloat[Burgers Convergence]{\includegraphics[width=1\linewidth]{images/roilqr plots/Convergence_burgers-1.png}}\\
      
      
\end{multicols}

\vspace{-1cm}
\begin{multicols}{3}
   
      \subfloat[Allen-Cahn]{\includegraphics[width=1\linewidth]{images/roilqr plots/AC_modes.png}}    
      \subfloat[Cahn-Hilliard]{\includegraphics[width=1\linewidth]{images/roilqr plots/CH_modes.png}}
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      \subfloat[Burgers]{\includegraphics[width=1\linewidth]{images/roilqr plots/burgers_modes.png}}\\
      
      
\end{multicols}

      
\caption{\small Convergence of Episodic cost for (a) Allen-Cahn, (b) Cahn Hilliard and (c) Viscous Burgers PDE (Top Row), and corresponding variation of number of modes for the 99.999\% energy cutoff with ILQR iteration (Bottom Row)}
% (Note that the `filtered' line in DDPG plots is the moving average over 10 episodes)%Bottom row: Terminal state MSE during testing in D2C vs DDPG. The solid line in the plots indicates the mean and the shade indicates the standard deviation of the corresponding metric.}
\label{d2c_2_training_testing}
% \vspace{-0.8cm}
\end{figure*}

\begin{table}[h]
%\begin{center}
\parbox{\linewidth}{
\caption{Comparison of the training outcomes of ILQR with the reduced order ILQR.}
\centering
\begin{tabular}{|c|c|c|}
\hline
& \multicolumn{2}{|c|}{\bf Training time (in sec.)}\\\cline{2-3}
{\bf PDE system} &{\bf ILQR} &{\bf roILQR}\\
\hline
{\bf Allen-Cahn($50 \times 50$)} &2292.38 &53.21 \\
\hline
%{\bf Goal-II(20X20)}&12327.36& 55.206 &4419.36*\\
{\bf Cahn-Hilliard($20 \times 20$)}&5295.21  &209.83\\
\hline
{\bf Viscous Burgers($100 \times 1$)} &146.99 &13.01\\
\hline

\end{tabular}
\label{d2c_comparison_table1}
\begin{tablenotes}
\item[1] The open-loop training is run on a laptop with a 2-core CPU@2.9GHz and 12GB RAM. No multi-threading at this point.
\end{tablenotes}
%\end{center}
}
\end{table}

\begin{table}[ht]
\vspace{-0.5cm}
\caption{Parameter size comparison for LTV system identification between ILQR and roILQR}
\label{parasize}
\centering
\vspace{0.1in}
\begin{threeparttable}
\setlength{\tabcolsep}{0.6mm}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
System& No. of  & No. of & No. of  &Dimensionality&Dimensionality\\
&steps&actuators&observed&for&for\\
&&($n_u$)&states($n_x$)& ILQR& roILQR\\
&&&&$ (n_x+n_u)$& $(l+n_u)$\\
\hline
Allen-Cahn& 10&4 &2500&2504 &7\\
\hline
Cahn-Hilliard& 10 &4& 400 &404&9\\
\hline
Burgers & 20&2 & 100&102 &9\\
\hline
\end{tabular}
}
\vspace{0.1in}
\end{threeparttable}
\label{params_comp}
\end{table}

\begin{figure}[!htpb]
\vspace{-0.3cm}
% \setlength{\belowcaptionskip}{-44pt}
\centering
\begin{multicols}{2}
    \subfloat[Initial state]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_int_0.png}}
    % \subfloat[Intermediate-I)]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_int_2.png}}
    \subfloat[Intermediate-I]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_1_3.png}}\\
         
      
\end{multicols}
% \vspace{-1cm}

\begin{multicols}{2}
      \subfloat[Intermediate-II]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_1_9.png}}
    %   \subfloat[Intermediate-IV]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_1_8.png}}
      \subfloat[Final State]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_2_10.png}}
      
      
\end{multicols}

% \begin{multicols}{2}
   
%     %   \subfloat[Intermediate-III]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_0_5.png}}
%       \subfloat[Intermediate-II]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_1_2.png}}
%       \subfloat[Final State]{\includegraphics[width=\linewidth]{images/roilqr plots/3d_2_6.png}}\\
      
      
% \end{multicols}
      
\caption{Optimal trajectory for the Cahn-Hilliard PDE.}
% (Note that the `filtered' line in DDPG plots is the moving average over 10 episodes)%Bottom row: Terminal state MSE during testing in D2C vs DDPG. The solid line in the plots indicates the mean and the shade indicates the standard deviation of the corresponding metric.}
% \vspace{-0.5cm}
\label{AC_traj}
\end{figure}


\begin{figure}
% \vspace{-0.5cm}
% \begin{multicols}{1}
   
\includegraphics[width=1\linewidth]{images/roilqr plots/burgers_traj-1.png}
      
      
% \end{multicols}

      
\caption{\small Optimal trajectory for the Burgers PDE.}
\label{bg_traj}
\end{figure}

\subsubsection{Repeatability/Variance in training}    
The plots in Fig. \ref{d2c_2_conv} show the mean and standard deviation of the cost curves when starting with different initial guesses, averaged over 100 runs. From this, we can see that the algorithm repeatedly converges to the same minima.

\subsubsection{Quality of the solution}    
% \textcolor{red}{Aren't the solutions the same now for both now?}
The plots in Fig. \ref{d2c_2_comp} compare the iterations of the full-scale ILQR vs the proposed reduced-order modification. 
We observe that the RO-ILQR converges to a solution with a cost within $14\%$ of the true optimal. This is in agreement with the convergence analysis we develop in Section \ref{analysis}, wherein we are guaranteed to converge to the set $S_\infty$. It is observed that this convergence bound is, in practice, tighter than the conservative estimate provided by the mathematical analysis. Moreover, the RO-ILQR approach is far cheaper computationally when compared to the full order ILQR. However, we also note that in the case of Burger's equation, the reduced order solution is almost of the same quality of the full order solution.
% We observe that both methods converge to the same true optimal solution. Furthermore, the RO-iLQR approach is far cheaper computationally when compared to the full order iLQR. 

\begin{figure}[!htpb]
\vspace{0.0cm}
\centering

\begin{multicols}{2}
   
      \subfloat[Allen-Cahn (GS-II)]{\includegraphics[width=1\linewidth]{images/roilqr plots/AC_roilqr_cost2.png}}
      \subfloat[Cahn-Hilliard (GS-I)]{\includegraphics[width=1\linewidth]{images/roilqr plots/CH_roilqr_cost2.png}}
      %/DDPG_Plots/ddpg_checkerboard_h_10_10000r.png}}
    %   \subfloat[Burgers Convergence\\(GS-III)]{\includegraphics[width=1\linewidth]{images/roilqr plots/CH_roilqr_cost2.png}}\\%FILLER
      
      
\end{multicols}
      
\caption{\small Convergence of Episodic cost for (a) Allen-Cahn, (b) Cahn Hilliard and (c) Viscous Burgers PDE averaged over 100 runs with different initial guesses}
\label{d2c_2_conv}
% \vspace{-0.05cm}
\end{figure}

\begin{figure}[!htpb]
\setlength{\belowcaptionskip}{-15pt}
% \vspace{-0.5cm}
\centering

\begin{multicols}{2}
   
      \subfloat[Allen-Cahn Comparison\\(GS-II)]{\includegraphics[width=1\linewidth]{figure/roilqr_AC_comp.pdf}}
    %   \subfloat[Cahn-Hilliard Comparison\\(GS-II)]{\includegraphics[width=1\linewidth]{images/roilqr plots/burgers_roilqr_comp.png}}%FILLER
    %   %/DDPG_Plots/ddpg_checkerboard_h_10_10000r.png}}
      \subfloat[Cahn-Hilliard Comparison\\(GS-I)]%\\(GS-III)]
      {\includegraphics[width=1\linewidth]{figure/roilqr_CH_comp.pdf}}\\%FILLER
      
      
\end{multicols}

\subfloat[Burgers Comparison]{\includegraphics[width=0.5\linewidth]{figure/roilqr_burgers_comp.pdf}}

\caption{\small Comparing convergence of Episodic cost for (a) Allen-Cahn and (b) Viscous Burgers PDE, starting from same initial guess}
\label{d2c_2_comp}
\end{figure}

% \begin{figure}
%     \centering
%     \import{figure/}{fig_L1.pdf_tex}
%     \caption{}
%     \label{fig}
% \end{figure}

\subsubsection{Comparison With Deep RL}
In order to benchmark our algorithm, we have previously compared a data-based implementation of the standard, full order ILQR algorithm with the Deep Deterministic Policy Gradient (DDPG) algorithm, for the Allen-Cahn and Cahn-Hilliard Equations discussed in Sec.~\ref{applications} \cite{material_control_journal}. It was observed that DDPG fails to converge to the target microstructure for the scale of the problems considered here, due to the overparametrization that stems from the increasing dimensionality of the resulting system. Thus, using DDPG or similar techniques to design a feedback law is infeasible in the context of such problems. Moreover, the structure of the DDPG algorithm, or similar model-free RL techniques in general, does not allow for the implementation of model order techniques that we implement in RO-ILQR, making the comparison unfair.



==> improvements.tex <==
\section{Improvement in system identification: Number of Rollouts}\label{sec_alg}

Intro to using LLS-CD to find $A_t$ and $B_t$ in the full vs reduced order model.

The system identification problem thus reduces from an $O(n_x+n_u)$ problem to $O(n_\alpha + n_u)$ problem, where $n_\alpha<< n_x$.



==> pde_introduction.tex <==
\subsection{Optimal Control Problems Studied}
\label{applications}

This section introduces the PDEs used for comparing the reduced order ILQR with the standard ILQR approach implemented on a full-order, high DOF system.

% The PDEs were spatio-temporally discretized using a Central-Difference scheme.
% \textcolor{red}{Get the equations out of inline below.}
\subsubsection{1D Viscous Burger's Equation}
Consider the viscous Burger's Equation:
\begin{equation*}
    \frac{\partial u}{\partial t}+u \frac{\partial u}{\partial x}=\nu \frac{\partial^2 u}{\partial x^2},
\end{equation*}
with external control inputs on the boundaries corresponding to blowing/suction such that $u(0,t)=U_1(t)$; $u(L,t)=U_2(t)$.


\subsubsection{Material Microstructure evolution - Allen-Cahn and Cahn-Hilliard Equation}
The evolution of material micro-structures can be represented by two types of partial differential equations, i.e., the Allen-Cahn (A-C) equation \cite{ALLEN19791085} representing the evolution of a  non-conserved quantity, and the Cahn-Hilliard (C-H) equation \cite{Cahn1958} representing the evolution of a conserved quantity. The Allen-Cahn equation has the general form %$\frac{\partial \phi}{\partial t}= -M(\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi),$ %\\
\begin{align}
    \frac{\partial \phi}{\partial t}= -M(\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi), %\label{eq:Dyn_main}
\end{align}
while the Cahn-Hilliard equation has the form %$\frac{\partial \phi}{\partial t}= \nabla \cdot M \nabla (\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi)$,
\begin{align}
    \frac{\partial \phi}{\partial t}= \nabla \cdot M \nabla (\frac{\partial F}{\partial\phi}-\gamma\nabla^{2}\phi), %\label{eq:Dyn_main}
\end{align}
where $\phi=\phi(x,t)$ is called the order parameter. In Controls parlance, $\phi$ is the state of the system, and is infinite dimensional. It reflects the component proportion of each phase of material system. For a two-phase system studied in this work, $\phi$ = -1 represents one pure phase and $\phi$ = 1 represent the other, while $\phi$ $\in$ (-1, 1) stands for a combination state of both phases on the boundary interface between two pure phases; \textit{M} is a parameter related to the mobility of material, which is assumed \textit{constant} in this study; \textit{F} is an energy function with a nonlinear dependence on $\phi$; $\gamma$ is a gradient coefficient controlling the diffusion level or thickness of the boundary interface.

In this study, we adopt the following general form of energy density function %\textcolor{blue}{Please give reference}:
\begin{align}
    F(\phi;T,h) = \phi^{4}+T\phi^{2}+h\phi . \,%\label{eq:D_well} 
\end{align}
Here, the parameters \textit{T} and \textit{h} are not governed by the A-C and C-H equations. Instead, they may be externally set to any value and may be spatially as well as temporally varying. 

% \subsection{Nonlinear Schrodinger's Equation}
% Insert NLS formulation
